SA6D: Self-Adaptive Few-Shot 6D Pose Estimator for Novel and Occluded Objects

To enable meaningful robotic manipulation of objects in the real-world, 6D pose estimation is one of the critical aspects. Most existing approaches have difficulties to extend predictions to scenarios where novel object instances are continuously introduced, especially with heavy occlusions. In this work, we propose a few-shot pose estimation (FSPE) approach called SA6D, which uses a self-adaptive segmentation module to identify the novel target object and construct a point cloud model of the target object using only a small number of cluttered reference images. Unlike existing methods, SA6D does not require object-centric reference images or any additional object information, making it a more generalizable and scalable solution across categories. We evaluate SA6D on real-world tabletop object datasets and demonstrate that SA6D outperforms existing FSPE methods, particularly in cluttered scenes with occlusions, while requiring fewer reference images.

==> docs/preliminaries.tex <==
\section{Preliminaries}
\label{preliminaries}
\begin{figure*}
\centering
	\includegraphics[width=\linewidth]{figs/segmentation_iccv.png}
		\caption{\textbf{Online self-adaptation module}. We first train a segmentor  $\varphi$ with synthetic data and consider it as a base model, which is applied afterwards on both reference and test images in real scenes to predict segmentations. Meanwhile, a copy of $\varphi$ will be updated in the next step to generate distinguishable target object representation, we call it adaptive segmentor $\varphi*$. With the ground-truth translation of the target object in the reference images $\textrm{T}_{\textrm{ref}}$, the object center can be reprojected to the image. For each reference image, the segment is selected from $\varphi$ as a positive sample if it includes the reprojected object center and the remaining segments as negative. An object-level representation is computed by averaging the pixel-wise dense features from $\varphi*$ for each segment predicted by $\varphi$. Consequently, we apply a contrastive loss over the positive and negative object representations and update $\varphi*$ iteratively. After adaptation, $\varphi*$ generates the target object representation $r*$ by averaging over all positive representations from reference images. Given a test image, we obtain the representation of candidates by averaging the dense features of $\varphi*$ segmented by $\varphi$. We subsequently compute the cosine similarity between each candidate and $r*$ and the most similar candidate is chosen as the segment of the target object. Meanwhile, the canonical object model and local reconstruction are computed based on the segments and depth images.}
		\label{fig:segmentation}
\end{figure*}

In this section, we present an overview of Gen6D\newcite{Gen6D} and highlight the key enhancements of our proposed method over Gen6D, which consists of three components, namely detector, selector, and refiner. Given RGB images, the detector initially identifies the target object in the test image by comparing the visual similarity between the patches of test image and the object-centric reference images cropped based on the known pose and object diameter. Afterwards, the detector outputs a score map based on the visual similarity along with a predicted region of interest (ROI).
Consequently, the selector selects the most similar reference image based on the predicted ROI and uses the reference pose as an initial guess, which will be updated by a learning-based refiner to obtain the final pose. However, since detector and selector rely purely on the visual similarity between test and reference images, Gen6D requires large and diverse reference images to cover the appearance of all different viewpoints and cannot deal with occlusions as the authors claimed. 
In contrast, SA6D solves the aforementioned problems by incorporating depth information to reveal the geometric features which are used to improve the scene understanding against occlusions. Notably, SA6D improves the efficiency with fewer reference images compared with Gen6D.

